Convolutional 2D Knowledge Graph Embeddings

Link prediction for knowledge graphs is the task of predicting missing relationships between entities. Previous work on link prediction has focused on shallow, fast models which can scale to large knowledge graphs. However, these models learn less expressive features than deep, multi-layer models -- which potentially limits performance. In this work, we introduce ConvE, a multi-layer convolutional network model for link prediction, and report state-of-the-art results for several established datasets. We also show that the model is highly parameter efficient, yielding the same performance as DistMult and R-GCN with 8x and 17x fewer parameters. Analysis of our model suggests that it is particularly effective at modelling nodes with high indegree -- which are common in highly-connected, complex knowledge graphs such as Freebase and YAGO3. In addition, it has been noted that the WN18 and FB15k datasets suffer from test set leakage, due to inverse relations from the training set being present in the test set -- however, the extent of this issue has so far not been quantified. We find this problem to be severe: a simple rule-based model can achieve state-of-the-art results on both WN18 and FB15k. To ensure that models are evaluated on datasets where simply exploiting inverse relations cannot yield competitive results, we investigate and validate several commonly used datasets -- deriving robust variants where necessary. We then perform experiments on these robust datasets for our own and several previously proposed models and find that ConvE achieves state-of-the-art Mean Reciprocal Rank across most datasets.

==> GNUmakefile <==
# GNU Makefile for LaTeX projects (papers, presentations, etc.), works fine
#	for projects where each TeX-file is self-contained (usually the case).
#
# Note: We assume that each TeX-file depends on all images and Bib-files, this
# 	is not ideal but is the safest choice unless you know a way to extract
# 	this information for the TeX-files (do tell me if you do, but I doubt it
# 	since TeX is Turing complete last time I checked).
#
# Author:		Pontus Stenetorp	<pontus stenetorp se>
# Version:		2013-05-14

TEX_FILES=${shell find -maxdepth 1 -name '*.tex' | xargs -n 1 -r basename}
TEX_BNAMES=${subst .tex,,${TEX_FILES}}
PDF_FILES=${subst .tex,.pdf,${TEX_FILES}}
BIB_FILES=${shell find -maxdepth 1 -name '*.bib' | xargs -n 1 -r basename}

LATEX_BIN=pdflatex
BIBSORT_SH=~/git/ppod/ext/bibsort/bibsort

# Drop your images into this directory (we do try to handle any necessary
# 	conversions).
IMAGE_DIR=graphics
SVG_IMAGES=${shell find '${IMAGE_DIR}' -name '*.svg'}
PDF_IMAGES=${subst .svg,.pdf,${SVG_IMAGES}}

# Goal(s) for converting SVG to PDF using Inkscape.
define svg2pdf-target
${2}: ${1}
	inkscape -z --file='${1}' --export-pdf='${2}' -D
endef
${foreach SVG_IMAGE,${SVG_IMAGES}, \
	${eval ${call svg2pdf-target,${SVG_IMAGE}, \
		${subst .svg,.pdf,${SVG_IMAGE}}} \
	} \
}

# Goal(s) for generating our final PDFs.
define pdf-target
${1}.blg: ${1}.tex ${BIB_FILES} ${PDF_IMAGES}
	${LATEX_BIN} '${1}'
	if grep '\\bibcite' '${1}.aux' || grep '\\citation' '${1}.aux'; \
	then \
		for _ in `seq 2`; \
		do \
			bibtex '${1}'; \
		done; \
	fi

${1}.pdf: ${1}.blg
	${LATEX_BIN} '${1}'
	for _ in `seq 2`; \
	do \
		if grep -i 'rerun' '${1}.log'; \
		then \
			${LATEX_BIN} '${1}.tex'; \
		fi; \
	done
endef
${foreach TEX_BNAME,${TEX_BNAMES}, \
	${eval ${call pdf-target,${TEX_BNAME}} \
	} \
}

.DEFAULT_GOAL=all
all: ${PDF_FILES}

# XXX: Not done...
#.PHONY: bibsort
#bibsort:
#trap "rm -f $${TMP}" INT TERM EXIT
#	find . -maxdepth 1 -name '*.bib' -exec sh -c \
#		"TMP=`mktemp` && cat {} | ${BIBSORT_SH} > $${TMP} && cat $${TMP} > {} && rm -f $${TMP}" \;
# TMP=`mktemp`; trap "rm -f ${TMP}" INT TERM EXIT; cat sture.bib | ~/git/ppod/ext/bibsort/bibsort > ${TMP}; cat ${TMP} > sture.bib; rm -f ${TMP}

.PHONY: clean
clean:
	for TEX_BNAME in ${TEX_BNAMES}; \
	do \
		for SUFFIX in aux bbl blg dvi idx lof log lot nav out pdf ps snm toc; \
		do \
			rm -f "$${TEX_BNAME}.$${SUFFIX}"; \
		done; \
	done
	rm -f ${PDF_IMAGES}
	find . -maxdepth 1 -name '*~' | xargs -r rm

